Toward transient finite element simulation of thermal deformation of machine tools in real-time

Finite element models without simplifying assumptions can accurately describe the spatial and temporal distribution of heat in machine tools as well as the resulting deformation. In principle, this allows to correct for displacements of the Tool Centre Point and enables high precision manufacturing. However, the computational cost of FEM models and restriction to generic algorithms in commercial tools like ANSYS prevents their operational use since simulations have to run faster than real-time. For the case where heat diffusion is slow compared to machine movement, we introduce a tailored implicit-explicit multi-rate time stepping method of higher order based on spectral deferred corrections. Using the open-source FEM library DUNE, we show that fully coupled simulations of the temperature field are possible in real-time for a machine consisting of a stock sliding up and down on rails attached to a stand.

==> modelproblem.tex <==
% !TEX root = paper.tex
\section{A model problem: stability and order of convergence}
\input{defsjw.tex}
We propose the following model problem.
%\todo{TODO: check sign}, $v_0-u(x,t)$ has a stable fix point at $u(x,t)=v_0$
\todo{We need to make the connection between the model problem and the full problem very clear and give a convincing demonstration of the model problem's usefulness.
Can we, may be, illustrate the following
\begin{itemize}
	\item stability limit for diffusion is $\Delta t = \mathcal{O}(\nu \Delta x^2)$, but accuracy requires only $\Delta  t = \mathcal{O}(\nu \Delta x)$?
	\item in contrast, for the moving part, both stability and accuracy require $\Delta t = \mathcal{O}(\Delta x/v)$?
	\item Also, would be good to show how MR-SDC produces one order per iteration.
\end{itemize}
if we can show this for the model problem, it would provide motivation for our splitting later.}

Consider the model problem
\todo{TODO: check sign}, $v_0-u(x,t)$ has a stable fix point at $u(x,t)=v_0$
\begin{equation}
	u_{t} = \nu u_{xx} + \alpha \left( v_0 -  u(x,t)  \right) \delta \left(x - a t \right)
\end{equation}
where the spatial domain is the interval $[0, 2\pi]\subset \realn{1}$ with periodic boundary conditions, i.e. $u:[0, 2 \pi] \times [0, T] \mapsin \real$.
Note, that all the derivations have to be understood in a distributional sense. Equality of expressions is  defined by the weak formulation.
Thus we can work with Fourier series which do not converge in a strong sense, but in a weak formulation.

We  expand the solution $u$  in a Fourier series
\begin{equation}
	u(x,t) = \frac{1}{2} a_0 + \sum_{k=1}^{\infty} a_k(t) \cos( k x) + b_k(t) \sin(k x)
\end{equation}
and use that the delta-Distribution has a weak convergent Fourier expansion
\begin{equation}
	\delta(x - a t) = \frac{1}{2 \pi} +  \frac{1}{\pi} \sum_{k=1}^{\infty} \cos(k a t) \cos(k x) + \sin(k a t) \sin(k x).
\end{equation}
Inserting
\begin{align*}
	\sum_{k=1}^{\infty} \dot{a}_k(t) \cos(k x) + \dot{b}_k(t) \sin( k x) &= \sum_{k=1}^{\infty} -\nu k^2 a_k(t) \cos(k x) - \nu k^2 b_k(t) \sin( k x)  \\
		& + \alpha v_0 \left( \frac{1}{2\pi} + \frac{1}{\pi} \sum_{k=1}^{\infty} \cos(k a t) \cos(k x) + \sin(k a t) \sin( k x) \right) \\
		& - \alpha \left( \frac{1}{2} a_0 + \sum_{k=1}^{\infty} a_k(t) \cos( k x) + b_k(t) \sin(k x) \right) \\
		&\cdot \left(  \frac{1}{2 \pi} +  \frac{1}{\pi} \sum_{k=1}^{\infty} \cos(k a t) \cos(k x) + \sin(k a t) \sin(k x) \right)
\end{align*}
...
For the constant mode we get
\begin{equation}
	\dot{a}_0 =  \frac{\alpha v_0}{2 \pi} - \frac{\alpha a_0}{4 \pi} \Rightarrow a_0(t) = c e^{-\frac{\alpha t}{4 \pi}} + 2 v_0.
\end{equation}
Eventually, after truncation at some $N$ and ignoring modes $\cos((N+1)x)$ and higher and collection coefficients of $\cos(kx)$ and $\sin(kx)$, this will lead to a system of equations
\begin{equation}
	\dot{a}_k = -\nu k^2 a_k(t) + \alpha v_0 f_k(t) + \alpha \left( \sum_{j=1}^{N} c_{k,j} a_{k}(t) + \sum_{j=1}^{N} d_{k,j} b_{k}(t) \right)
\end{equation}
and
\begin{equation}
	\dot{b}_k = -\nu k^2 b_k(t) + \alpha v_0 g_k(t) + \alpha \left( \sum_{j=1}^{N} e_{k,j} a_{k}(t) + \sum_{j=1}^{N} g_{k,j} b_{k}(t) \right).
\end{equation}
In compact matrix notation this reads
\begin{equation}
	\begin{bmatrix} \dot{a}_0 \\ \dot{\ve{a}} \\ \dot{\ve{b}} \end{bmatrix} =  - \nu \begin{bmatrix} 0 & 0 & 0 \\ 0 & \matr{S} & 0 \\ 0 & 0 & \matr{S} \end{bmatrix} 
	\begin{bmatrix} a_0 \\ \ve{a} \\ \ve{b} \end{bmatrix} 
	- \alpha \begin{bmatrix} -1/4\pi & 0 & 0 \\ \matr{C} & \matr{D} & \matr{E} \\ \matr{E} & \matr{F} & \matr{H} \end{bmatrix} \begin{bmatrix} a_0 \\ \ve{a} \\ \ve{b} \end{bmatrix} 
	+ \alpha v_0 \begin{bmatrix} 1/2\pi \\  \ve{f} \\ \ve{g} \end{bmatrix}.
\end{equation}
Maple provides an easy way to compute the entries of $\ve{C}$, $\ve{D}$, $\ve{E}$, $\ve{F}$, $\ve{G}$ and $\ve{H}$.
\begin{align}
\left(\begin{array}{cccc} \dot{a}_0 \cr \dot{a}_1 \cr \dot{a}_{2} \cr \dot{b}_1 \cr \dot{b}_2 \end{array}\right) =& -\nu \left(\begin{matrix} 0 & 0 & 0 & 0 & 0 \cr 0 & 1 & 0 & 0 & 0 \cr 0 & 0 &4 &  0 & 0 \cr 0 & 0 & 0 &1 & 0 \cr 0 &0 & 0 & 0 & 4\end{matrix} \right)\left(\begin{array}{c} a_0 \cr {a}_1 \cr {a}_{2} \cr {b}_1 \cr {b}_2 \end{array}\right) \cr
		 -&\alpha \input{coefficientMatrix_2}\left(\begin{array}{c}a_0 \cr  {a}_1 \cr {a}_{2} \cr {b}_1 \cr {b}_2 \end{array}\right) \cr
	+& \alpha \frac{v_0}{\pi}\left(\begin{array}{c} \frac{1}{2} \cr \cos(at) \cr \cos(2at) \cr \sin(at) \cr \sin(2at) \end{array}\right)
\end{align}
The eigenvalues of the full matrices with up to four modes and $\alpha=1$ and the eigenvalues of the coupling block matrices are
\begin{itemize}
 \item $N=2$:
  \begin{align}
    \input{eigenvalueFull_2}\,,  
    \input{eigenvalue_2}
  \end{align}
 \item $N=3$:
  \begin{align}
    \input{eigenvalueFull_3}\,,
    \input{eigenvalue_3}
  \end{align}
 \item $N=4$:
  \begin{align}
    \input{eigenvalueFull_4}\,,
    \input{eigenvalue_4}
  \end{align}
\end{itemize}
It is quite interesting, that none of the eigenvalues depend on time!
\todo{\begin{itemize}
       \item remove the imaginary parts. with python/sympy, they vanish on symbolic level
       \item the not so nice feature are the positive eigenvalues
      \end{itemize}}

\begin{figure}
	\centering
	\caption{Stability domains of MR-SDC (left) and Rosenbrock method (right).}
\end{figure}

\begin{figure}
	\centering
	\caption{Convergence of MR-SDC (left) and Rosenbrock method (right).}
\end{figure}

